Adaptive TTL-Based Caching for Content Delivery

Content Delivery Networks (CDNs) deliver a majority of the user-requested content on the Internet, including web pages, videos, and software downloads. A CDN server caches and serves the content requested by users. Designing caching algorithms that automatically adapt to the heterogeneity, burstiness, and non-stationary nature of real-world content requests is a major challenge and is the focus of our work. While there is much work on caching algorithms for stationary request traffic, the work on non-stationary request traffic is very limited. Consequently, most prior models are inaccurate for production CDN traffic that is non-stationary. We propose two TTL-based caching algorithms and provide provable guarantees for content request traffic that is bursty and non-stationary. The first algorithm called d-TTL dynamically adapts a TTL parameter using a stochastic approximation approach. Given a feasible target hit rate, we show that the hit rate of d-TTL converges to its target value for a general class of bursty traffic that allows Markov dependence over time and non-stationary arrivals. The second algorithm called f-TTL uses two caches, each with its own TTL. The first-level cache adaptively filters out non-stationary traffic, while the second-level cache stores frequently-accessed stationary traffic. Given feasible targets for both the hit rate and the expected cache size, f-TTL asymptotically achieves both targets. We implement d-TTL and f-TTL and evaluate both algorithms using an extensive nine-day trace consisting of 500 million requests from a production CDN server. We show that both d-TTL and f-TTL converge to their hit rate targets with an error of about 1.3%. But, f-TTL requires a significantly smaller cache size than d-TTL to achieve the same hit rate, since it effectively filters out the non-stationary traffic for rarely-accessed objects.

==> abstractToN.tex <==
Content Delivery Networks (CDNs) deliver a majority of the user-requested content on the Internet, including web pages, videos, and software downloads.  A CDN server caches and serves the content requested by users. Designing caching algorithms that {\em automatically} adapt to the heterogeneity, burstiness, and non-stationary nature of real-world content requests is a major challenge and is the focus of our work. While there is much work on caching algorithms for stationary request traffic, the work on non-stationary request traffic is very limited. Consequently, most prior models are inaccurate for production CDN traffic that is non-stationary. We propose two TTL-based caching algorithms and provide provable guarantees for content request traffic that is bursty and non-stationary. The first algorithm called d-TTL dynamically adapts a TTL parameter using a stochastic approximation approach.  Given a feasible target hit rate, we show that the hit rate of d-TTL converges to its target value for a general class of bursty traffic that allows Markov dependence over time and non-stationary arrivals. The second algorithm called f-TTL uses two caches, each with its own TTL. The first-level cache adaptively filters out non-stationary traffic, while the second-level cache stores frequently-accessed stationary traffic. Given feasible targets for both the hit rate and the expected cache size, f-TTL asymptotically achieves both targets. We implement d-TTL and f-TTL and evaluate both algorithms using an extensive nine-day trace consisting of 500 million requests from a production CDN server.  We show that both d-TTL and f-TTL converge to their hit rate targets with an error of about 1.3\%. But,  f-TTL requires a significantly smaller cache size than d-TTL to achieve the same hit rate, since it effectively filters out the non-stationary traffic for rarely-accessed objects.


==> table3.tex <==
\begin{table*}[!ht]
\small
\caption{\s{Impact of exponential changes in constant step size $\eta$ on the performance of d-TTL (robustness analysis of d-TTL).}}
\label{tab:d-ttl-rob}
\centering
\begin{tabular}{|p{0.55in}|p{0.55in}|p{0.55in}|p{0.55in}|p{0.55in}|p{0.55in}|p{0.55in}|p{0.55in}|p{0.55in}|p{0.55in}|}
\hline
Target  & \multicolumn{3}{|c|}{Average OHR (\%)} & \multicolumn{3}{|c|}{Average cache size (GB)} & \multicolumn{3}{|c|}{5\% outage fraction}  \\
\cline{2-10}
 OHR (\%) & $\eta$ = 0.1 & $\eta$ = 0.01 & $\eta$ = 0.001 & $\eta$ = 0.1 & $\eta$ = 0.01 & $\eta$ = 0.001 & $\eta$ = 0.1 & $\eta$ = 0.01 & $\eta$ = 0.001 \\
\hline 
\hline
60 & 59.35 & 59.36 & 59.17 & 9.03 & 6.00 & 5.41 & 0.01 & 0.01 & 0.05 \\
\hline
80 & 79.13 & 78.72 & 77.69 & 150.56 & 97.67 & 75.27 & 0.07 & 0.11 & 0.23 \\
\hline
\end{tabular}
\end{table*}

\begin{table*}[!ht]
\small
\caption{\s{Impact of linear changes in constant step size $\eta=0.01$ on the performance of d-TTL (sensitivity analysis of d-TTL).}}
\label{tab:d-ttl-sen}
\centering
\begin{tabular}{|p{0.55in}|p{0.55in}|p{0.55in}|p{0.55in}|p{0.55in}|p{0.55in}|p{0.55in}|p{0.55in}|p{0.55in}|p{0.55in}|}
\hline
Target  & \multicolumn{3}{|c|}{Average OHR (\%)} & \multicolumn{3}{|c|}{Average cache size (GB)} & \multicolumn{3}{|c|}{5\% outage fraction}  \\
\cline{2-10}
 OHR (\%) & $\eta$(1+0.05) & $\eta$ & $\eta$(1-0.05) & $\eta$(1+0.05) & $\eta$ & $\eta$(1-0.05) & $\eta$(1+0.05) & $\eta$ & $\eta$(1-0.05) \\
\hline 
\hline
60 & 59.36 & 59.36 & 59.36 & 5.98 & 6.00 & 6.02 & 0.01 & 0.01 & 0.01 \\
\hline
80 & 78.73 & 78.72 & 78.71 & 98.21 & 97.67 & 97.1 & 0.11 & 0.11 & 0.11 \\
\hline
\end{tabular}
\end{table*}

\begin{table*}[!ht]
\small
\caption{\s{Impact of exponential changes in constant step size $\eta_s$ on the performance of f-TTL (robustness analysis of f-TTL).}}
\label{tab:f-ttl-rob}
\centering
\begin{tabular}{|p{0.55in}|p{0.55in}|p{0.55in}|p{0.55in}|p{0.55in}|p{0.55in}|p{0.55in}|p{0.55in}|p{0.55in}|p{0.55in}|}
\hline
Target  & \multicolumn{3}{|c|}{Average OHR (\%)} & \multicolumn{3}{|c|}{Average cache size (GB)} & \multicolumn{3}{|c|}{5\% outage fraction}  \\
\cline{2-10}
 OHR (\%) & $\eta_s$ = 1e-8 & $\eta_s$ = 1e-9 & $\eta_s$ = 1e-10 & $\eta_s$ = 1e-8 & $\eta_s$ = 1e-9 & $\eta_s$ = 1e-10  & $\eta_s$ = 1e-8 & $\eta_s$ = 1e-9 & $\eta_s$ = 1e-10  \\
\hline 
\hline
60 & 59.36 & 59.36 & 59.36 & 5.46 & 2.96 & 1.88 & 0.01 & 0.01 & 0.02 \\
\hline
80 & 78.65 & 78.55 & 78.47 & 89.52 & 55.08 & 43.34 & 0.12 & 0.14 & 0.17 \\
\hline
\end{tabular}
\end{table*}

\begin{table*}[!ht]
\small
\caption{\s{Impact of linear changes in constant step size $\eta_s=\text{\normalfont 1e-9}$ on the performance of f-TTL (sensitivity analysis of f-TTL).}}
\label{tab:f-ttl-sen}
\centering
\begin{tabular}{|p{0.55in}|p{0.55in}|p{0.55in}|p{0.55in}|p{0.55in}|p{0.55in}|p{0.55in}|p{0.55in}|p{0.55in}|p{0.55in}|}
\hline
Target  & \multicolumn{3}{|c|}{Average OHR (\%)} & \multicolumn{3}{|c|}{Average cache size (GB)} & \multicolumn{3}{|c|}{5\% outage fraction}  \\
\cline{2-10}
 OHR (\%) & $\eta_s$(1+0.05) & $\eta_s$ & $\eta_s$(1-0.05) & $\eta_s$(1+0.05) & $\eta_s$ & $\eta_s$(1-0.05) & $\eta_s$(1+0.05) & $\eta_s$ & $\eta_s$(1-0.05) \\
 \hline 
\hline
60 & 59.36 & 59.36 & 59.36 & 3.01 & 2.96 & 2.91 & 0.01 & 0.01 & 0.01 \\
\hline
80 & 78.55 & 78.55 & 78.54 & 55.65 & 55.08 & 54.27 & 0.14 & 0.14 & 0.14 \\
\hline
\end{tabular}
\end{table*}
